Unified Embodied VLM Reasoning with Robotic Action via Autoregressive Discretized Pre-training

General-purpose robotic systems operating in open-world environments must achieve both broad generalization and high-precision action execution, a combination that remains challenging for existing Vision-Language-Action (VLA) models. While large Vision-Language Models (VLMs) improve semantic generalization, insufficient embodied reasoning leads to brittle behavior, and conversely, strong reasoning alone is inadequate without precise control. To provide a decoupled and quantitative assessment of this bottleneck, we introduce Embodied Reasoning Intelligence Quotient (ERIQ), a large-scale embodied reasoning benchmark in robotic manipulation, comprising 6K+ question-answer pairs across four reasoning dimensions. By decoupling reasoning from execution, ERIQ enables systematic evaluation and reveals a strong positive correlation between embodied reasoning capability and end-to-end VLA generalization. To bridge the gap from reasoning to precise execution, we propose FACT, a flow-matching-based action tokenizer that converts continuous control into discrete sequences while preserving high-fidelity trajectory reconstruction. The resulting GenieReasoner jointly optimizes reasoning and action in a unified space, outperforming both continuous-action and prior discrete-action baselines in real-world tasks. Together, ERIQ and FACT provide a principled framework for diagnosing and overcoming the reasoning-precision trade-off, advancing robust, general-purpose robotic manipulation. Project page: https://geniereasoner.github.io/GenieReasoner/

==> section/tokenizer.tex <==
\section{Method}
\label{tokenizer}


\subsection{Preliminaries}
A central challenge in developing Vision-Language-Action (VLA) models lies in the representation of the action space.
These systems are trained on diverse demonstration datasets $\mathcal{D}$ with the objective of mapping robot observations, such as images $I \in \mathbb{R}^{H\times W\times3}$, and a high-level user instruction, $l$, to a sequence of continuous actions $a_{1:H} \in \mathcal{A}$, where $\mathcal{A}$ denotes the continuous action space. 
Current approaches typically fall into one of two ways.

One line of work discretizes the action space, enabling the use of powerful autoregressive models that treat actions as tokens. These methods have demonstrated a strong ability to adhere to complex language instructions~\cite{pertsch2025fast}.
In contrast, another way models actions as continuous distributions, often leveraging diffusion models to generate high-precision and smooth motor commands. 
This dichotomy presents a fundamental trade-off: discrete representations excel at semantic grounding and long-horizon planning, while continuous representations offer superior motor control fidelity.

To bridge this gap, we propose to learn a compact, discrete representation of actions by training a specialized tokenizer. Our approach is based on a diffusion autoencoder framework, consisting of an encoder $\mathcal{E}_\theta$ and a decoder $\mathcal{D}_\theta$, that learns a mapping between continuous action chunks and a discrete latent codebook. 
The encoder, $\mathcal{E}_\theta$, maps a continuous action chunk $a$ to a discrete latent code $c \in \{1, \dots, K\}$. The decoder, $\mathcal{D}_\theta$, then reconstructs the action chunk conditioned on this code.

Both the encoder and decoder are implemented using a transformer-based architecture. Crucially, to handle the complex, multimodal nature of robot actions, the decoder $\mathcal{D}_\theta$ is trained to model the reconstruction distribution $p(a|c)$ using a Rectified Flow objective. The entire tokenizer is optimized end-to-end on the demonstration dataset $\mathcal{D}$. This process yields a discrete action space suitable for high-level planning, while the Rectified Flow decoder ensures that these discrete codes map back to high-fidelity, continuous motor commands.


\subsection{Disco Action Tokenizer}
The Discrete-Contiguous Action Tokenizer (DiscoAT) is a vector-quantized autoencoder (VQ-AE) featuring an encoder, $\mathcal{E}_\theta$, and a diffusion-based decoder, $\mathcal{D}_\theta$. 
The architectural backbone for both components is a multimodal diffusion transformer, configured to process sequences with a patch size of one.
The tokenization process commences with an action chunk, which is first standardized via normalization to yield $a_{1:H} \in \mathbb{R}^{H \times S}$. The encoder $E$ then maps this normalized input to a continuous latent representation $e \in \mathbb{R}^{L \times D}$, performing temporal ($L \leq H$) and spatial ($D \leq S$) compression.
% no necessary to compress spatial
This continuous representation is then quantized into a discrete code $c \in \mathbb{R}^{L \times D}$ by mapping each vector in $e$ to its nearest neighbor in a learned codebook containing $V$ prototype vectors.
The final stage involves the diffusion decoder $D$, which learns to reverse a forward noising process to reconstruct the original normalized actions. Conditioned on the discrete code $c$, the decoder is trained to iteratively denoise a standard Gaussian noise vector over a series of timesteps, ultimately generating a reconstruction of $a_{1:H}$.

As shown in Figure x, the initial latent codes $c_{ini} \in R^{L\times D}$, which are all zeroes, will produce the final latent token by interacting with features of $a_{1:H}$.
\begin{equation}
    e = \mathcal{E}_\theta(a_{1:H}, c_{ini}),
\end{equation}
$e$ will be quantized by a bitwise quantizer following lookup-free quantization, getting $c$ as shown below:
\begin{equation}
    c_k = \mathcal{Q}(e_k) = \operatorname{sign}(e_k).
\end{equation}
The decoder, denoted by $\mathcal{D}_\theta$, is trained to reconstruct the original action chunk. The reconstruction is conditioned on the discrete code $c$ and an input noise vector $z \sim \mathcal{N}(0, I)$. The model parameters $\theta$ are optimized using the Rectified Flow objective. The decoder's prediction is formulated as:
\begin{equation}
    a_{\text{pred}} = \mathcal{D}_\theta(z, c).
\end{equation}

\subsubsection{Training Loss}
Following \cite{magvit_v2}, we apply an entropy loss and a commitment loss to train the quantization process. The combined quantization loss, $\mathcal{L}_q$, is formulated as:
\begin{equation}
\mathcal{L}_{\text{entropy}} = \mathbb{E}\big[H(\mathcal{Q}(e) \big] - H(\mathbb{E}\big[\mathcal{Q}(e)\big] ), 
\end{equation}
\begin{equation}
\mathcal{L}_{\text{commit}} = \mathbb{E} \bigg[ \big\|e - \mathcal{Q}(e) \big\|_2^2 \bigg].
\end{equation}

We train the decoder network, $\mathcal{D}_\theta$, using the Rectified Flow objective~\cite{liu2022flow}. The goal is to learn the velocity field of a simple, straight-line trajectory that transports samples from a noise distribution to the data distribution. This trajectory is defined by a linear interpolation $a_t = (1-t)z + ta$ for $t \in [0, 1]$, where $a$ is the target action data. The corresponding constant velocity of this path is simply $v = a - z$.

The flow-matching loss is formulated as a simple mean-squared error objective:
\begin{equation}
\mathcal{L}_{\text{flow}} = \mathbb{E}_{a, z, t}\left[ \left\| (a - z) - \mathcal{D}_\theta(a_t, c, t) \right\|_2^2 \right],
\end{equation}
where the condition $c$ is the quantized latent code from the encoder, i.e., $c = \mathcal{Q}(\mathcal{E}_\theta(a, c_{ini}))$. Architecturally, the time step $t$ is passed to the MMDit blocks of the decoder via AdaLN modulation to produce time-dependent velocity predictions.

\subsection{Disco VLA}
With the pre-trained Disco Action Tokenizer in place, we now introduce the complete Vision-Language-Action policy, which we term Disco VLA.
This policy, which is based on a pre-trained VLM, operates entirely in the discrete action space learned by our tokenizer, leveraging the strengths of autoregressive modeling for long-horizon, language-conditioned tasks. 
The overall training process is divided into two sequential stages.

\paragraph{Stage 1: Action Space Discretization}
First, we leverage the trained encoder $\mathcal{E}_\theta$ and quantizer $\mathcal{Q}$ of our Disco Action Tokenizer. We process the entire continuous action dataset $\mathcal{D}$ to create a new, corresponding dataset of discrete action codes, $\mathcal{D}_c = \{ (I, l, c) \}$.
Each continuous action chunk $a$ in the original dataset is mapped to its discrete latent code $c = \mathcal{Q}(\mathcal{E}_\theta(a, c_{ini}))$.
This offline tokenization step provides the supervision signal for training our policy model.

\paragraph{Stage 2: Autoregressive Policy Training}
The Disco VLA policy, denoted as $\pi_\phi$, is an autoregressive, transformer-based model. It takes as input the robot's visual observation $I$ and the language instruction $l$, and is trained to predict the sequence of discrete action codes $c$ from the dataset $\mathcal{D}_c$. The model is optimized by minimizing the negative log-likelihood of the ground-truth code sequence, which is a standard cross-entropy loss for classification:
\begin{equation}
\mathcal{L}_{\text{policy}} = \mathbb{E}_{(I, l, c) \sim \mathcal{D}_c} \left[ -\sum_{i=1}^{L} \log \pi_\phi(c_i | c_{<i}, I, l) \right].
\end{equation}
By modeling the task in this discrete space, the policy's optimization is decoupled from the generative process of the tokenizer. Consequently, the policy is trained with a standard cross-entropy loss, avoiding the direct influence of the diffusion objective.

\paragraph{Inference}
At inference time, the robot receives an observation $I$ and a language instruction $l$. The Disco VLA policy $\pi_\phi$ is then unrolled autoregressively to generate a sequence of predicted discrete codes $\hat{c}$. 
Predicted code $\hat{c}$ will be fed into the pre-trained decoder $\mathcal{D}_\theta$ of our disco action tokenizer. 
The decoder reconstructs the corresponding continuous action chunk $\hat{a} = \mathcal{D}_\theta(z, \hat{c})$, which is then executed by the robot. 
This two-step process---predicting in the discrete latent space and decoding to the continuous action space---allows our system to combine the semantic grounding of discrete models with the high-fidelity motor control of our Rectified Flow decoder.

\subsection{Cotraining with Embodied Understanding Data}
While general-purpose Vision-Language Models (VLMs) have demonstrated remarkable capabilities, they often lack the nuanced understanding required for embodied AI, particularly in areas like fine-grained spatial perception and hierarchical task planning.
To address this gap, we curate a supplementary dataset specifically designed to bolster these abilities, thereby enhancing the overall embodied intelligence of our agent.

==> table/aer.tex <==
\begin{table*}
\centering
\caption{The 15 sub-tasks in the AgiBot Embodied Reasoning benchmark, categorized into four core capability dimensions.}
\label{tab:aer_tasks}
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{llll}
\toprule
\textbf{Perception \& Understanding} & \textbf{Planning \& Reasoning} & \textbf{Mistake Handling} & \textbf{Collaboration} \\
\midrule
\texttt{Scene Understanding} & \texttt{Subtask Planning} & \texttt{Mistake Existence} & \texttt{Human Intention Comprehension} \\
\texttt{Relative Position Grounding} & \texttt{Success Detection} & \texttt{Mistake Classify} & \texttt{Human-Robot Interaction} \\
\texttt{Task Grounding} & \texttt{Reasoning} & \texttt{Mistake Recovery} & \\
\texttt{Dualview Matching} & \texttt{Action Understanding} & & \\
 & \texttt{Trajectory Understanding} & & \\
 & \texttt{Task Progress} & & \\
\bottomrule
\end{tabular}%
}
\hspace{-10mm}
\end{table*}
